DanModCap: Designing a Danmaku Moderation Tool for Video-Sharing Platforms that Leverages Impact Captions with Large Language Models

Online video platforms have gained increased popularity due to their ability to support information consumption and sharing and the diverse social interactions they afford. Danmaku, a real-time commentary feature that overlays user comments on a video, has been found to improve user engagement, however, the use of Danmaku can lead to toxic behaviors and inappropriate comments. To address these issues, we propose a proactive moderation approach inspired by Impact Captions, a visual technique used in East Asian variety shows. Impact Captions combine textual content and visual elements to construct emotional and cognitive resonance. Within the context of this work, Impact Captions were used to guide viewers towards positive Danmaku-related activities and elicit more pro-social behaviors. Leveraging Impact Captions, we developed DanModCap, an moderation tool that collected and analyzed Danmaku and used it as input to large generative language models to produce Impact Captions. Our evaluation of DanModCap demonstrated that Impact Captions reduced negative antagonistic emotions, increased users' desire to share positive content, and elicited self-control in Danmaku social action to fostering proactive community maintenance behaviors. Our approach highlights the benefits of using LLM-supported content moderation methods for proactive moderation in a large-scale live content contexts.

==> 06-findings.tex <==
\begin{CJK*}{UTF8}{gbsn}

\section{Findings}
We begin by presenting viewers’ perception of generative Impact Captions in terms of cognitive and emotional resonance and examining the interplay between textual and non-textual elements within these captions. The second section delves into an exploration of user understanding and engagement, extending beyond social and community activism to encompass user attention, community dynamics, and video platforms. In the final section, we describe related moderation practices.

\subsection{Perception of Generative Impact Captions}

\subsubsection{Perceived Cognitive Resonance} 
Our research findings suggest that viewers’ cognitive resonance with Impact Captions stems primarily from their comprehension of the underlying intent in the captions’ creation. This comprehension is rooted in shared experiences and articulated intentions. Impact Captions effectively encapsulate viewer thought processes, attitudes, and intentional responses to diverse Danmaku stimuli.


\paragraph{Alignment with viewers' thoughts, experience, and intended activism} 
A predominant segment of the viewer (P2-P11, and P13) reported a heightened understanding of Impact Captions, attributing this to a congruence between the content of the captions and their thoughts, attitudes, and intentions, particularly in viewing Danmaku-enhanced videos. This Alignment fostered a deeper connection and resonance with their experiences and inclinations. For instance, viewer P9 remarked, \textit{``Having followed LOL games extensively, I am intimately familiar with the discourse in Danmaku. When Impact Captions echoed sentiments about a player's subpar performance, it resonated deeply, reflecting a comprehension of the perspective of an e-sports aficionado.''} This perception persisted across viewers (P12) with varying online socialization preferences.

Furthermore, viewers identified with Impact Captions that mirrored their own opinions or values, reinforcing their connection to the content. viewer P4 noted: \textit{``Observing unanimous Danmaku praise in vloggers' videos and contributing similar comments creates a shared atmosphere. In these instances, I perceive the Impact Captions as reflecting a similar disposition and sense of belonging to a common community.''}  Additionally, viewers (P10) highlighted that Impact Captions often articulated desires they harbored but had not expressed, providing an alternative avenue for online expression, as indicated by viewer P1 \textit{``I do not usually like to express myself online, but Impact Captions is kinda like a representative that can speak for me online.''}

\paragraph{Interpreting Textual Elements in Impact Captions} 
Regarding the textual dimension of Impact Captions, all viewers demonstrated awareness of the captions’ purpose and the context of their emergence. viewer P3, for example, commented on the potency and appeal of the "Humoristic-Tsukkomi style" finding it particularly impactful. She said, ``\textit{This expression [Humoristic-Tsukkomi style]is so powerful and interesting, it is too funny. (P3)''}
 Contrastingly, some viewers, like P8, perceived the tone of certain captions as mechanical and rigid. There was also a sentiment, as expressed by viewer P1, that certain types of Impact Captions lacked distinctiveness, particularly in terms of textual features. For example, viewer P1 stated, \textit{``I understand the point of the text depictions, but I did not find anything special or different. Maybe the only difference is the length because these are all shown in the video. Maybe except for the different color and shape underneath, from a textual aspect, I did not find these Impact Captions to be different.''}

\subsubsection{Perceived Emotional Resonance} 
Viewers in this study predominantly experienced emotional resonance through the Impact Captions, particularly when these captions displayed emotions congruent with their own. viewers (P4, P7, P9 and P13) often found themselves vicariously expressing emotions through these captions. For example, viewer P9 shared discomfort when encountering derogatory online messages against a favored team, yet found solace in the Impact Captions’ empathetic response. As they expressed, \textit{``When I see messages online taunting and calling names to a team I support after they lose a game, it makes me uncomfortable. However, Impact Captions seemed to understand my emotions and responded to the others.''}
The study also observed that some viewers (P2, P7 and P15) were inclined to ascribe their knowledge and emotions to Impact Captions, notably influenced by the persuasive power of their visual elements. The interpretation of emotions was often guided by the visual cues of the captions, such as the shape and color of speech bubbles in the “Humoristic-Tsukkomi style” which some viewers associated with feelings of anger and repulsion towards provocative Danmaku. For example, viewer p9 mentioned, \textit{``There were instances when I was furious at what the Danmaku were saying and was about to retaliate, but then the Impact Captions also appeared and expressed their disapproval, making me feel that they were just as disgusted as I was with the others' comments.''}


\subsection{Engaging and Understanding with \textit{DanModCap} System}
This section elucidates the dynamics of viewers’ engagement and comprehension of the DanMod- Cap system. It emphasizes changes in viewers’ attention, sense of community connection, and heightened awareness of video platforms’ ability to utilize user data for content generation. This encompasses an exploration of the system’s influence on shaping public opinion and the viewers’ cognizance of their social impact and responsibilities.

\subsubsection{The Dynamics of Viewer Attention} \label{attentionchange}
We identified a dynamic shift in viewers’ attention, attributable to the presence of Impact Captions. Indeed, viewers were initially drawn to the Danmaku content, oftentimes at the expense of primary video content. However, the introduction of Impact Captions gradually fostered a realignment of their focus either towards the captions or back toward the video. This is particularly prominent in the context of explanatory captions, which motivated viewers against overindulgence in Danmaku. The words of viewer P2 exemplified this shift: \textit{``I have actually forgotten what this video is for, you know, I think it is fine to listen to the voiceover of the video is all, the Danmaku is much more exciting, so I am mostly going to watch the content of the Danmaku and not pay attention to the video screen because the screen is not that important, I think. This Impact Captions popping up to tell me what the video is about is fine; if it is something I am interested in and I missed it, I will rewind and go back to check it out.''}  A subset of viewers also reported that Impact Captions could divert their attention towards Danmaku content. viewer P4 noted: \textit{``Initially I was unaware of what was going on with Danmaku, paying attention to see [the video creator] in make-up and explaining, and suddenly noticed what the Impact Captions were saying inside  `注意言辞，尊重他人 (Pay attention to words and respect others.)', and I paused to see what they were fighting about.''}

\subsubsection{Sense-making of Community Cohesion}
Our findings suggest that viewers experienced a heightened sense of community cohesion, characterized by belonging, companionship, and security.

\paragraph{Sense of Belongingness}
We observed that certain linguistic constructs within Impact Captions transformed into a distinct and flexible language adopted by the viewer P4, P9 and P13. This linguistic adoption played a crucial role in cultivating a sense of group belonging and shared interests. The Impact Captions' capability to reflect viewers' emotions and perceptions contributed significantly to reinforcing this sense of belonging. viewer P13 remarked, \textit{``For example, I have seen the King of Thieves video written to appear ``感谢凯多老师！ (Thank you, Kaido-sensei!).'' , `恭喜路飞新帝(Congratulations to Luffy Shindei!)' When I see the Danmaku video, I feel that it[Impact Captions] and I are both secondary characters who also watch anime and understand us and that everyone swipes such Danmaku.''}

\paragraph{Sense of Companionship}
Most viewers expressed a belief that Impact Captions created an illusion of shared viewership, even in solitary viewing contexts. This effect was amplified by the captions’ humorous and explanatory nature. As Viewer P4 expressed, \textit{"The Impact Captions felt like a like-minded friend, accompanying and interacting with me throughout the video."}

\paragraph{Sense of Security}
Several viewers (P1, P7 and P9) reported a sense of resonance when Impact Captions articulated their unspoken thoughts or emotions, and expressed that this enhanced their sense of security within the wider community. Viewer P9’s comment illustrated that the Impact Captions provided a voice for her unexpressed thoughts, reducing the anxiety of potential online backlash and offering protection. She explained \textit{``There are times when I am afraid to post messages on Danmaku for fear of being cyber-bullied, especially by some fans. However, this[Impact Captions] makes me relax my stress, like an alternative to my expression, instead of expressing myself on a public platform, with the feeling of being protected.''}

\subsubsection{Implications for Societal Ethos in Video Platforms Utilizing genAI}
We found some viewer (P1, P2,P13 and P14) consensus on the societal responsibilities of video platforms, especially those employing generative AI technologies. Content on these platforms, ranging from entertainment to user-generated material, mirrors and—potentially—molds societal culture and values. Danmaku often serves as a forum for social discourse, influencing public consciousness and attitudes. The genAI-enabled Impact Captions can subtly guide viewer behavior by endorsing positive Danmaku interactions or critiquing negative ones. viewer P1 reflected, \textit{``The deployment of Impact Captions carries inherent social responsibility. These captions do more than convey information; they steer Danmaku trends. Positive captions can foster a constructive viewing atmosphere, whereas negative or sarcastic use might deteriorate it. Hence, platforms with such capabilities must exercise discretion in their generative use, considering the broader impact on the online environment.''}

\subsection{Viewer Practices of \textit{DanModCap} System}

\subsubsection{Self-Reflection on Danmaku Language Usage}
We found that some viewers (P7, P9 and P12) spontaneously self-reflected on the speech patterns and word choices they used in Danmaku. This introspection was primarily triggered by the perception that the generated Impact Captions magnified negative emotions and remarks, adversely affecting the viewing experience for others. For instance, viewer P12 thought that the Impact Captions seemed to be responding directly to his Danmaku message, prompting a reevaluation of his contributions. He reflected, \textit{``I would feel like that Impact Caption was there to troll me like another user saw my Danmaku and came over to remind me.''}

\subsubsection{Emotional Self-Regulation and Resilience}
viewers (P3,P4,, P5, P7, and P14) reported that they deployed strategies for emotional self-regulation as a reaction to Impact Captions, particularly during heightened emotional fluctuation. While viewers generally exhibited tolerance and restraint towards offensive or irrelevant Danmaku content, prolonged exposure to such content—and particularly those that involved personal insults—frequently provoked strong emotional responses. In these instances, Impact Captions served as a proxy for viewers’ reactions, alleviating stress and facilitating emotional equilibrium. 
As an illustration, when viewers encountered derogatory Danmaku, they perceived Impact Captions as a means of counter-expression, helping to alleviate their irritation and providing a sense of solidarity. In this context, Impact Captions serve as catalysts for emotional self-control during this process. viewer P7 illustrated this neatly: \textit{``I am very uptight sometimes like that Danmaku kept saying that that blogger was unattractive, it is just a life attack. I get furious at that kind of thing, and the word `舔 (lick),' which girls especially hate, is very erotic, but a verb the system does not recognize as a sensitive word, so it cannot be blocked. Nevertheless, at this point, Impact Captions is like a way to help me fight against those Danmaku, or maybe I am not the only one who resents it. The mood was much better all of a sudden.''} 
 Moreover, some viewers noted that Impact Captions helped reorient their focus from Danmaku to video content, especially when encountering explanatory captions (as discussed in \autoref{attentionchange}).

\subsubsection{Transformation of the Sharing and Debating Desire}
We found that Impact Captions influenced viewers’ inclination to share and express opinions, fostering a more proactive approach to moderation. A reduced engagement in provocative, conflicting, or negative discussions characterized this shift. Several viewers (P3,P7) adapted their participation in Danmaku; some reduced their frequency of comments as Impact Captions echoed their sentiments, while others transformed their originally negative or confrontational comments into positive contributions. P3 commented, \textit{``When Impact Captions articulate my thoughts, I no longer feel compelled to express them separately.''} Similarly, P8 and P13 thought that Impact Captions steered them toward more positive interactions, prompting them to delete negative messages and contribute constructively. As P8 said: \textit{``I realized that the impact captions are trying to guide me, to make me do something else. To relieve my negative emotions, I will delete the negative message or something that people would not like I want to share and respond to the call of the Impact Captions, either going back to watching videos or just copying the roasting content said by the Impact Captions, it is really funny, to liven up the atmosphere.''}


\subsubsection{Spontaneous Maintaining an Online Environment}
The affirmative nature of Impact Captions inspired several viewers and actively supported constructive Danmaku content. This included mounting Danmaku flows, echoing positive comments, and encouraging engagement with video content. Some viewers (P8, P11, P13, and P14) spontaneously contributed to fostering a healthy online discourse, particularly resonating with the positive community culture reflected in the Impact Captions. As P6 stated, \textit{``I make a conscious effort to maintain a positive tone in Danmaku, focusing discussions on video-related topics and employing neutral language to initiate new conversations.''}
While another viewer explained, ``I wanted to mimic the behavior of that Impact Captions, it made me feel like I wasn't alone in trying to be nice and talk normally online. (P11)''


\end{CJK*}





